Harmony-Aware Music-driven Motion Synthesis with Perceptual Constraint on UGC Datasets

With the popularity of video-based user-generated content (UGC) on social media, harmony, as dictated by human perceptual principles, is critical in assessing the rhythmic consistency of audio-visual UGCs for better user engagement. In this work, we propose a novel harmony-aware GAN framework, following a specifically designed harmony evaluation strategy to enhance rhythmic synchronization in the automatic music-to-motion synthesis using a UGC dance dataset. This harmony strategy utilizes refined cross-modal beat detection to capture closely correlated audio and visual rhythms in an audio-visual pair. To mimic human attention mechanism, we introduce saliency-based beat weighting and interval-driven beat alignment, which ensures accurate harmony score estimation consistent with human perception. Building on this strategy, our model, employing efficient encoder-decoder and depth-lifting designs, is adversarially trained based on categorized musical meter segments to generate realistic and rhythmic 3D human motions. We further incorporate our harmony evaluation strategy as a weakly supervised perceptual constraint to flexibly guide the synchronized audio-visual rhythms during the generation process. Experimental results show that our proposed model significantly outperforms other leading music-to-motion methods in rhythmic harmony, both quantitatively and qualitatively, even with limited UGC training data. Live samples 15 can be watched at: https://youtu.be/tWwz7yq4aUs

==> Sec/backups.tex <==
Such evaluation is targeted as a problem of measuring the rhythmic consistency between audio and visual sequences based on beats. To enhance the approximation of human perception in the assessment, we analyze the consistent audio-visual beat detection and include an attention mechanism in our interval-driven beat alignment.

To analyze the effectiveness of the proposed harmony loss


\acknowledgments{
This work was supported by TCL Research America through Interactive Hyperstory project.}



The rest of the paper is organized as follows. We provide a brief review of the current literature for audio-visual evaluation and audio-driven motion synthesis in Section 2. Section 3 provides details for beat detection and alignment in our harmony evaluation mechanism. In Section 4, we present the proposed meter-driven adversarial framework with the detailed network architecture and the harmony-aware hybrid loss function. The implementation and experimental results are demonstrated in Section 5. Finally we draw our conclusions in Section 6.


To handle the difficulty of cross-modal synthesis, following the literature \cite{tang2018dance,ren2020self} the encoder-decoder structure is utilized for the feature translation between sequences to sequences. Considering the chronological order in the data sequences, recurrent structures are introduced into the architecture of encoder and decoder in order to obtain features with temporal correlations. The Gated Recurrent Units (GRUs) \cite{chung2014empirical}), as a typical structure of RNN, has been confirmed to outperform the common Long Short Term Memory (LSTM) structure in sequence learning for its fewer parameters and reduced computation. Similarly to previous work \cite{lee2019dancing,ren2020self}, our music-to-motion generator G consists of a GRU-based audio encoder and pose decoder, demonstrated in the left part of Fig \ref{NetArch}. 

In addition, differently from analyzing only the audio features, we concatenate it with our initial pose features to enhance the cross-modal learning in our decoder. The skip connections are also applied to intentionally add those audio-visual features into the future layers. Since our generator $G$ is aimed at producing human motions in 3D poses, it is more difficult to accurately estimate the additional depth dimension compared to synthesizing 2D motions. Inspired by the 2D-to-3D lifting for the depth analysis in image and video processing \cite{tome2017lifting,Luo2020VideoDepth,kopf2020one}, we estimate the 2D poses first and construct the depth lifting branch to produce the 3D poses based on the 2D estimation. Taking advantage of the similarity between the 2D and 3D poses, the depth can be efficiently generated.


\begin{table}[htbp]
\centering
\caption{Comparision of realism}
\label{table_realism}
\begin{tabular}{c c c c c}

\hline
Model Name & MSE & CosineDis & LPIPS & FID \\ \hline
HarmoGAN w/o $\pazocal{L}_{harmo}$ & 0.2007	& 0.3478 & 0.0299 & 12.24 \\ 
HarmoGAN & \textbf{0.0314} & \textbf{0.1183} & \textbf{0.0150} & \textbf{8.64} \\ 

\end{tabular}
\end{table}


In Fig. \ref{abl_mq}, the lower the values of all metrics the better. We can see that the realism of the synthesized movements is improved significantly under the evaluation of point-level, sequence-level, and feature-level metrics when $\pazocal{L}_{harmo}$ is incorporated. The relatively small size of our training set can result in overfitting and missing the global minimum when descending gradients during the network learning. However, with the guidance from $\pazocal{L}_{harmo}$, such a weak supervision is able to benefit the training and make our model achieve a better convergence, which can explain the increased performance shown in Table \ref{table_realism}.  



The methods in \cite{lee2019dancing,ren2020self} are tested with their published codes and pretrained models. The evaluation results of quantified harmony and hit rate of music beats are demonstrated in Tables \ref{quantiharmo} and \ref{hitrate-ab} with details for the 7 types of dance music. They show that our HarmoGAN outperforms the other models distinctly with respect to both metrics. Referring to the testing results on the Dance dataset (see Table \ref{dance_avh}), the lower performance of our baseline HarmoGAN without $\pazocal{L}_{harmo}$ implies that it overfits on the limited amount of training samples when tested on the Ballroom dataset \cite{gouyon2006experimental}, while guided by the weakly-supervised harmony loss our HarmoGAN is able to alleviate such problem and maintain good performance on different testing datasets.
  
   
Compared with the baseline HarmoGAN without $\pazocal{L}_{harmo}$, in \cite{ren2020self} the proposed GCN-based pose loss and the self-attention cross-modal discriminator may intrinsically benefit the harmonization. They regularize the hierarchical representations of skeletons in the generated motions to make them consistent with the extracted musical features. However, such improvement lacks robustness and is highly affected by the bias of dance types in the training dataset. The post-processing beat warper in \cite{lee2019dancing} can relatively lift the performance evenly but is still limited. Differently from the other models, during the motion synthesis our HarmoGAN can directly produce distinct and robust improvements for the audio-visual harmony independent of the dance types.


When it comes to the performance of human dancer, in the previous work such as \cite{lee2019dancing}, due to the inappropriate visual beat detection and the lack of considering the influence of human attention, it is difficult for the ground-truth professional dancer to perform well in the evaluation of cross-media harmony. Differently, under our improved evaluation mechanism, the human dancer can hit around 75\% of the music beats, which is more reasonable than the work in \cite{lee2019dancing} providing around 50\% of the hit rate.

When it comes to the performance of human dancer, it does not achieve the optimal situation with respect to the hit rate of audio beats, which is similar to findings of \cite{lee2019dancing}. Differently, our proposed evaluation mechanism refines the strategy of visual beat detection and takes the influence of human attention into consideration. Such improvements are also used to adjust the calculation details of hit rate, where the professional human dancer here can hit around 75\% of the music beats, which is much more reasonable in practice than the work in \cite{lee2019dancing} providing around 50\% of the hit rate.


As mentioned in \cite{lee2019dancing,ren2020self}, the training sets of the other two models are around 60 times and 5 times more than ours, respectively, which contributes to richer motion representation in the testing results compared with HarmoGAN.


In this paper, we propose a harmony-aware GAN framework to tackle the audio-driven motion synthesis. In order to generate motions harmonious with the given music, we dive deep into the audio-visual correlation under human perception and propose a novel evaluation mechanism that can achieve better cross-domain beat alignment. Due to the advantage of synthesis by analysis, such mechanism is then converted into a harmony loss function and incorporated into the model as a weakly-supervised regularizer. The experimental results show that with the assistance of the harmony loss, our model can provide significant improvements in audio-visual harmony compared with other state-of-the-art models. Meanwhile, the proposed evaluation mechanism can be verified that it is basically consistent with human perception and effective in reflecting the perceptual audio-visual harmony. 



==> Sec/conclu.tex <==
\section{Conclusion}

In this paper, we propose a harmony-aware GAN framework \tred{\sout{to tackle the audio-driven motion synthesis}}\tblue{for synthesizing audio-driven motions}. In order to generate motions harmonious with \tred{\sout{the}}\tblue{a} given music, we first dive deep into the correlation between audio and visual signals that affect\tred{\sout{s}} human perception. A novel evaluation mechanism is then proposed to quantify the audio-visual harmony based on cross-domain beat alignment. In order to reflect the perceptual harmony in a more accurate way, we refine the beat detection strategy and introduce human attention rules into our method. \tred{\sout{By}}\tblue{Upon} doing so, our harmony evaluation mechanism \tred{\sout{is}}\tblue{becomes} not only sensitive to the unsynchronization between an audio-visual beat pair\tblue{,} but also takes the saliency of beat\tblue{s} into consideration. In cooperation with \tred{\sout{the}}\tblue{a} training framework driven by \tred{\sout{the usage of}}\tblue{a} musical meter, \tred{\sout{such}}\tblue{the} mechanism is converted into a harmony loss function and incorporated into the model as a weakly-supervised regularizer to guide the motion synthesis. Additionally, our model \tred{\sout{also benefits}}\tblue{is also benefited} from adversarial learning with the aid of two discriminators that constrain cross-modal and spatio-temporal consistency\tred{\sout{, respectively}}. The experimental results show that our final HarmoGAN model can output human movement sequences with good motion quality based on \tred{\sout{relatively a}}\tblue{a relatively} small training dataset. Furthermore, our model \tred{\sout{provides significant improvements in}}\tblue{can significantly improve} audio-visual harmony\tblue{, both quantitatively and qualitatively,} compared with other state-of-the-art models\tred{\sout{ both quantitatively and qualitatively}}, which accordingly verifies the effectiveness of the harmony loss. 


\section*{APPENDIX}
\section*{A. Interface for User Study}

In \tred{\sout{the main}}\tblue{this} paper, we conduct two user studies in the \tred{\sout{experiments}}\tblue{experimental section}. \tred{\sout{One}}\tblue{The first user study} (in Section 5.4) is to \tred{\sout{tell}}\tblue{verify} whether our proposed harmony evaluation mechanism is consistent with human perception. The other \tred{\sout{one}}\tblue{user study} (in Section 5.5.3) qualitatively compares our generated results with \tblue{those of} several state-of-the-art models. As shown in Fig. \ref{userIF}, we visualize \tblue{some} screenshots of the interfaces that we develop\tblue{ed} for these studies. 


\begin{figure*}[ht]
\centerline{\includegraphics[scale=0.1]{fig/us.png}}
\caption{Examples of our user study interface. The part \tred{\sout{of}}\tblue{in} (a) is designed for \tblue{the} user study in Section 5.4\tblue{,} while \tblue{that in} (b) is \tblue{designed} for \tblue{for the user study in} Section 5.5.3. In (a)\tblue{,} the survey focuses more on the perceptual harmony between \tred{\sout{the}} audio and visual signals. In (b), participants are asked to consider the overall quality of the human motion video. The order of the samples in each test group \tred{\sout{are}}\tblue{is} shuffled randomly in order to avoid psychological inertia. }
\label{userIF}
\end{figure*}




